Using LLMs to Facilitate Formal Verification of RTL

Formal property verification (FPV) has existed for decades and has been shown to be effective at finding intricate RTL bugs. However, formal properties, such as those written as SystemVerilog Assertions (SVA), are time-consuming and error-prone to write, even for experienced users. Prior work has attempted to lighten this burden by raising the abstraction level so that SVA is generated from high-level specifications. However, this does not eliminate the manual effort of reasoning and writing about the detailed hardware behavior. Motivated by the increased need for FPV in the era of heterogeneous hardware and the advances in large language models (LLMs), we set out to explore whether LLMs can capture RTL behavior and generate correct SVA properties. First, we design an FPV-based evaluation framework that measures the correctness and completeness of SVA. Then, we evaluate GPT4 iteratively to craft the set of syntax and semantic rules needed to prompt it toward creating better SVA. We extend the open-source AutoSVA framework by integrating our improved GPT4-based flow to generate safety properties, in addition to facilitating their existing flow for liveness properties. Lastly, our use cases evaluate (1) the FPV coverage of GPT4-generated SVA on complex open-source RTL and (2) using generated SVA to prompt GPT4 to create RTL from scratch. Through these experiments, we find that GPT4 can generate correct SVA even for flawed RTL, without mirroring design errors. Particularly, it generated SVA that exposed a bug in the RISC-V CVA6 core that eluded the prior work's evaluation.

==> txt/2.background.tex <==
\section{Background and Motivation}\label{sec:background}

\subsection{Formal Property Verification (FPV)}
% Methodology: industry separate engineers. Creativity of LLM is an opportunity
% Talk about industry standards for formal verification.
% Formal Verif of comparing modules is not as useful since it requires to have the module already or create a model.


SystemVerilog Assertions (SVA)~\cite{sva_spec} can express temporal relations over RTL signals, which fall into two major classes: safety and liveness properties.
\textit{Safety} properties specify that “nothing bad will happen”, e.g. if A then B; while \textit{liveness} specify that “something good will happen”, e.g. if A eventually B.
FPV tools~\cite{jg_user,symbiotic} use solver engines based on formal methods to exhaustively search for counterexamples (CEXs) or proof.
FPV is the most thorough approach to verify hardware designs, but people are often feel discouraged to use it because of the steep learning curve and additional effort required to write assertions~\cite{formal_book}.
it has a steep learning curve and necessary engineering effort precludes designers from using it in practice~\cite{formal_book}.

% METHODOLOGY:
% -Modules are verified at unit level, properties are generated.
% -Make sure the interface assumptions are crystal clear!!
% -Properties are evaluated while running at system-level.

% For conciseness, for the rest of the paper when we refer to SVA we mean the SVA properties.
% And we use assertions and SVA interchangeably, although SVA also includes assumptions and covers.

% Define design verification (DV)

\subsection{Prior work at Generating SVA}

Much work done for domains like memory consistency models.
But this is to check the correctness of the design, wrt to the contract of memory consistency.
But we need a more general approach, to fill the gaps for the rest of the design.
% To be clear, for those domains where existing tools can help you automatize formal verification, you are probably better of using that.
% However, existing tools still require you to know how to use them, and they often require significant user input.
% The charm of language models is that they offer an easy to use interface, and can do many different tasks.

% LITERATURE: BlueSpec? Should we just use LLMs to generate BlueSpec?
% Use LLM to generate AutoSVA-compliant interfaces!

% We are going to re-use AutoSVA's FPV testbench (FT) generation flow.
% We do not need to provide RTL annotations to do that, but simply the path to the RTL.
% This generates an empty FT (without assertions), which we can populate with the help of the LLM.
% If we annotate the module interface, we can also obtain liveness assertions from AutoSVA, which we are going to do to compare coverage of the assertions generated by the LLM and AutoSVA, to find whether they are complementary.

% Although In the light of heterogenous computing, we have more unique hardware components.
% Since we have had much computing increase in the past decades, formal verification runtimes have become shorter, and applying formal verification to hardware designs is becoming more feasible.
% Pain points of formal verification:
% - Expertise in Formal Methods (steep learning curve)
% - Extra work to write the assertions
% LLMs can help with that. Private tutoring for formal verification.
% It helps create the formal specification, and also the assertions.
% on open-source projects

% Go Beyond Toy examples, can it actually help to develop real hardware?
% Can LLM re-implement Hardware, and then we compare them as equivalence checking? maybe timing is not right.


% AutoSVA: this paper introduced automatically generated end-to-end liveness properties of transactions between RTL modules and some safety properties about the transaction when multiple outstanding ones are allowed.
% However, it does not generate safety properties about the correctness of those transactions, as these often require the knowledge of the functionality of the module.
% In the light of LLMs, this paper wants to re-think a collaborative approach between humans and LLMs to generate formal specifications and assertions for hardware designs.

% Cite the Privia WACI paper as source, and also their references!






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Hardware designers can employ SVA properties for Test-Driven-Development (TDD), where CEXs help to refine the design~\cite{sutherland2015}. Moreover, this can be applied at early stages of RTL module development by using unit-level FV~\cite{tdd_formal}. However, FV's steep learning curve and necessary engineering effort preclude designers from using it in practice~\cite{formal_book}.
% \textbf{\proj democratizes FV for hardware designers and makes TDD practical by automating a key component of the FV problem: \textit{liveness and safety of module interfaces}.} 
% Instead of aiming to support functional FV, which is very implementation-dependent, \proj focuses on verifying that modules interact through \textit{well-formed transactions}. This verification entails checking certain attributes over the control logic involved in transactions and mapping them to properties that ensure that every module makes progress (does not hang). 

